Adaptive Quasi-Newton and Anderson Acceleration Framework with Explicit Global (Accelerated) Convergence Rates

Despite the impressive numerical performance of the quasi-Newton and Anderson/nonlinear acceleration methods, their global convergence rates have remained elusive for over 50 years. This study addresses this long-standing issue by introducing a framework that derives novel, adaptive quasi-Newton and nonlinear/Anderson acceleration schemes. Under mild assumptions, the proposed iterative methods exhibit explicit, non-asymptotic convergence rates that blend those of the gradient descent and Cubic Regularized Newton's methods. The proposed approach also includes an accelerated version for convex functions. Notably, these rates are achieved adaptively without prior knowledge of the function's parameters. The framework presented in this study is generic, and its special cases includes algorithms such as Newton's method with random subspaces, finite-differences, or lazy Hessian. Numerical experiments demonstrated the efficiency of the proposed framework, even compared to the l-BFGS algorithm with Wolfe line-search.

==> checklist.tex <==
\section*{Checklist}

 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [No]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [No]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Yes]
   \item The license information of the assets, if applicable. [No]
   \item New assets either in the supplemental material or as a URL, if applicable. [Yes]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}

==> detail_algo.tex <==
\section{Rethinking From Scratch Quasi-Newton Methods.} \label{sec:detail_construction_algo}


\subsection{First Ingredient: Subspace Approximation} 

Minimizing the upper bound \cref{eq:ineq_function} is costly in high dimension, as this requires an eigenvalue decomposition of the Hessian $\nabla^2 f(x)$ \citep{nesterov2006cubic}. Instead, let $D_t$ be some $N\times d$ matrix of directions (the construction of $D_t$ will be defined later in \cref{sec:direction_requirements}). By constraining the update $x_{t+1}-x_t$ in the span of directions $D_t$, i.e., 
\begin{equation}\label{eq:def_next_iterate}
    x_{t+1} = x_t + D_t\alpha_t,
\end{equation}
where $\alpha_t$ is a vector of $N$ coefficients, the minimization problem simplifies into
\[
    \alpha_{t} =\textstyle  \argmin_{\alpha\in\mathbb{R}^N} f(x_t) + \nabla f(x_t)D_t\alpha + \frac{1}{2}(D_t\alpha)^T\nabla^2 f(x_t)D_t\alpha + \frac{L}{6}\|D_t\alpha\|^3.
\]
The complexity of minimizing this upper bound is only $O(N^2d + N^3)$ operations, where $N$ is the number of columns of $D_t$ (see \cref{sec:solving_subproblem}).


\subsection{Second Ingredient: Multisecant Approximation of the Hessian} 

Typically, (limited-memory) quasi-Newton methods approximate the Hessian using the properties of the \textit{secant equation},
\[
    \nabla^2 f(x_i)(x_i-x_{i-1}) \approx \nabla f(x_i)-\nabla f(x_{i-1}),
\]
for the last $N$ pairs of iterates. Usually, the updates are done recursively, i.e., by updating an approximation of the Hessian one secant equation at a time. 

Instead, this paper approximates the Hessian using all the secant equations at once. Let the directions $D_t$ and their associated normalized gradient difference $G_t$ be defined as
\begin{align}\label{def:matrices_2}
    D_t = \left[\frac{y^{(t)}_1-z^{(t)}_1}{\|y^{(t)}_1-z^{(t)}_1\|_2},\ldots, \frac{y^{(t)}_N-z^{(t)}_N}{\|y^{(t)}_N-z^{(t)}_N\|_2}\right],\quad G_t = \left[\ldots,\frac{\nabla f(y^{(t)}_i)-\nabla f(z^{(t)}_i)}{\|y^{(t)}_i-z^{(t)}_i\|_2},\ldots\right].
\end{align}
where the points $y^{(t)}_i$, $z^{(t)}_i$ are defined as follow:
\begin{align}\label{def:matrices}
    Y_t = [y_1^{(t)},\ldots, y_N^{(t)}],\quad Z_t = [z_1^{(t)},\ldots, z_N^{(t)}].
\end{align}
For instance, l-BFGS uses $Y_t = [x_{t-N},\ldots, x_{t-1}]$ and $Z_t = [x_{t-N+1},\ldots, x_{t}]$ (which will \textbf{not} be the case in this paper, see \cref{sec:direction_requirements}). Intuitively, the matrix $G_t$ is a finite difference approximation of the Hessian-matrix product $\nabla^2f(x)D$. More precisely, the next theorem states a bound on the approximation error of this product as a function of the \textit{error vector} $\varepsilon_t$,
\begin{align} \label{eq:error_vector}
    \varepsilon_t \defas [e^{(t)}_1,\ldots,e^{(t)}_N], \quad \text{and} \quad e^{(t)}_i \defas \|y_i^{(t)}-z_i^{(t)}\| + 2\|z^{(t)}_i-x\|.
\end{align}
\begin{restatable}{theorem}{thmboundsecantalpha}\label{thm:bound_secant_alpha} Let the function $f$ satisfy \cref{assump:lipchitiz_hessian}. Let the matrices $D,\,G$ be defined as in \cref{def:matrices} and vector $\varepsilon$ as in \cref{eq:error_vector}. 
Then, for all $w\in\mathbb{R}^d$ and $\alpha\in\mathbb{R}^N$
\begin{align}
    \textstyle -\frac{L\|w\|}{2} |\alpha|^T\varepsilon_t\leq w^T(\nabla^2f(x)D_t-G_t)\alpha &\leq  \textstyle \frac{L\|w\|}{2} |\alpha|^T\varepsilon_t, \label{eq:bound_hessian_scalar}\\
    \|w^T(\nabla^2f(x)D_t-G_t)\| &\leq  \textstyle \frac{L\|w\|}{2} \|\varepsilon_t\|. \label{eq:bound_hessian_dalpha}
\end{align}
\end{restatable}
\paragraph{Proof sketch} The detailed proof can be found in \cref{sec:missing_proofs}. The main idea of the proof is as follows. From \cref{eq:ineq_secant} with $y=y_i$ and $z=z_i$, and \cref{assump:lipchitiz_hessian},  ($\cdot^{(t)}$ is removed for clarity),
\[
    \frac{\|\nabla f(y_i)-\nabla f(z_i)-\nabla^2f(x)(y_i-z_i)\|}{\|y_i-z_i\|} \leq \frac{L}{2}\|y_i-z_i\| + \|\nabla^2f(x)-\nabla^2f(z)\| \leq \frac{L}{2}e_i.
\]
The \textit{first} term in $e_i$ bounds the error of \cref{eq:ineq_secant}, while the \textit{second} comes from the distance between  \cref{eq:ineq_secant} and the current point $x$ where the Hessian is estimated. Then, it suffices to combine the inequalities with coefficients $\alpha$ to obtain \cref{thm:bound_secant_alpha}.

\subsection{Third Ingredient: Objective Function and Gradient Norm Upper bounds}


Since the approximation error between $\nabla^2 f(x) D$ and $G$ can be explicitly bounded, by carefully replacing the term $\nabla^2 f(x) D\alpha$ in \cref{eq:ineq_function,eq:ineq_secant} by $G\alpha$, alongside with an appropriate regularization, leads to the \textbf{type-I} and \textbf{type-II} bounds.

\begin{restatable}{theorem}{thmupperboundalgo} \label{thm:upper_bound_algo} Let the function $f$ satisfy \cref{assump:lipchitiz_hessian}. Let $x_{t+1}$ be defined as in \cref{eq:def_next_iterate}, the matrices $D_t,\,G_t$ be defined as in \cref{def:matrices} and $\varepsilon_t$ be defined as in \cref{eq:error_vector}. Then, for all $\alpha\in\mathbb{R}^N$,
\begin{align}
    & \textstyle  f(x_{t+1}) \leq f(x_t) + \nabla f(x_t)^TD_t\alpha + \frac{\alpha^TH_t\alpha}{2} + \frac{L\|D_t\alpha\|^3}{6}, \tag{Type-I bound}\label{eq:type1_bound}\\
    & \textstyle \|\nabla f(x_{t+1})\| \leq \left\|\nabla f(x_t) + G_t\alpha\right\| + \frac{L}{2}\Big( |\alpha|^T \varepsilon_t + \|D_t\alpha\|^2\Big), \tag{Type-II bound} \label{eq:type2_bound}
\end{align}
where $H_t \defas  \frac{G_t^TD_t+D_t^TG_t + \mathrm{I}L\|D_t\|\|\varepsilon_t\|}{2}$.
\end{restatable}
The proof can be found in \cref{sec:missing_proofs}. Minimizing \cref{eq:type1_bound,eq:type2_bound} leads to \cref{alg:type1,alg:type2}, {respectively}, whose constant $L$ is replaced by a parameter $M$, found by backtracking line-search. Type-I methods often refer to algorithms that aim to minimize the function value $f(x)$, while in contrast, type-II methods minimize the gradient norm $\|\nabla f(x)\|$ \citep{fang2009two,zhang2020globally,canini2022direct}. See \cref{alg:type1,alg:type2} for the implementation details.


\paragraph{Solving the sub-problems} In \cref{alg:type1,alg:type2}, the coefficients $\alpha$ are computed by solving a minimization sub-problem in $O(N^3+Nd)$ ( \cref{sec:solving_subproblem}), where $N$ is much smaller than $d$.
\begin{itemize}
    \item \textbf{ In \cref{alg:type1}}, the subproblem can be solved easily by a convex problem in two variables, which  involves an eigenvalue decomposition of the matrix $H \in\mathbb{R}^{N\times N}$  \citep{nesterov2006cubic}.
    \item \textbf{In \cref{alg:type2}}, the subproblem can be cast into a linear-quadratic problem of $O(N)$ variables and constraints that can be solved efficiently with SDP solvers (e.g., \texttt{SDPT3}).
\end{itemize}


\paragraph{Link with qN updates and Anderson Acceleration} \cref{alg:type1,alg:type2} are strongly related to known quasi-Newton methods and Anderson Acceleration technique, see \cref{sec:what_qn_method_do}.


\subsection{Fourth Ingredient: Direction Update Rules} \label{sec:direction_requirements}

One critical theoretical property in the analysis is how the gradient $\nabla f(x_t)$ is aligned with the directions $D_t$. Since $D_t$ is part of the algorithm design, a careful update can ensure that $D_t$ satisfy interesting theoretical properties.

% \subsubsection{Design Requirements}

Below are some assumptions on how to update $Y_t,\,Z_t,\,D_t$, called \textbf{requirements}. While not overly restrictive, naive methods such as keeping only previous iterates will not satisfy those.

All convergence results rely on \emph{one} of these conditions on the projector onto $\textbf{span}(D_t)$,
\begin{align}
    \textstyle P_t \defas D_t(D_t^TD_t)^{-1}D_t^T. \label{def:p_projector}
\end{align}
\begin{requirement}{1a}\label{assump:random_projector}
    For all $t$, the projector $P_t$  of the stochastic matrix $D_t$ satisfies $\mathbb{E}[P_t] = \frac{N}{d}\textbf{I}$.
\end{requirement}
\begin{requirement}{1b} \label{assump:projector_grad}
    For all $t$, the projector $P_t$ satisfies $P_t \nabla f(x_t) = \nabla f(x_t)$.
\end{requirement}
The first condition guarantees that, in expectation, the matrix $D_t$ spans partially the gradient $\nabla f(x_t)$, since $\mathbb{E}[P_t\nabla f(x_t)] = \frac{N}{d}\nabla f(x_t)$. The second condition requires the possibility to move towards the current gradient when taking the step $x+D\alpha$.

In addition, it is required that the norm of $\|\varepsilon_t\|$ does not grow too quickly, hence the next assumption.

\begin{requirement}{2}\label{assump:bounded_epsilon}
    For all $t$, the relative error $\frac{\|\varepsilon_t\|}{\|D_t\|}$ is bounded by $\delta$.
\end{requirement}
The \cref{assump:bounded_epsilon} is also non-restrictive, as it simply prevents taking secant equations at $y_i-z_i$ and $z_i-x_i$ too far apart. Most of the time, $\delta$ satisfies the crude bound $\delta \leq O(\|x_0-x^\star\|)$.

Finally, the condition number of the matrix $D$ also has to be bounded.
\begin{requirement}{3}\label{assump:bounded_conditionning}
    For all $t$, the matrix $D_t$ is full-column rank,i.e., $D_t^TD_t$ is invertible. In addition, its condition number $\kappa_{D_t} \defas \sqrt{\|D_t^TD_t\|\|(D_t^TD_t)^{-1}\|}$ is bounded by $\kappa$.
\end{requirement}
It is possible to ensure the condition with $\kappa=1$ if the directions are orthogonal.


\subsubsection{"Orthogonal Forward Estimate Only" Update Rule (Recommended)}

The \textit{"Orthogonal Forward Estimate Only"} update maintains $D_t$ orthonormal, i.e., $D_t^TD_t = I$ for all $t$, while ensuring that $\nabla f(x_t)$ belongs to the span of columns of $D_t$ (see \cref{alg:forward_estimate}). Those condition are satisfied thanks to an intermediate iterate $x_{t+\frac{1}{2}}$ that will be used to estimate $\nabla^2 f(x_t)\nabla f(x_t)$, which is called the \textbf{orthogonal forward estimate},
\[
    x_{t+\frac{1}{2}} = x_t - h\left(\nabla f(x_t)- \tilde D_{t-1} \left(\tilde D_{t-1}^T \nabla f(x_t)\right)\right), 
\]
where $h>0$ is a small stepsize, and $\tilde D_{t-1}$ is simply the matrix $D_{t-1}$ whose first column has been removed if its number of columns equals $N$. This forward estimate corresponds to a step of gradient descent projected onto the orthogonal space spanned by the columns of $\tilde D_{t-1}$. This projection step is cheap since the orthogonality of $D_t$ is maintained over the iterations.

After computing the forward estimate, it suffices to update the matrices $Y_t$, $Z_t$ as, respectively, a moving history of the previous forward iterates and previous iterates,
\[
    Y_t = [x_{t-N+\frac{3}{2}},\ldots,x_{t+\frac{1}{2}}],\qquad Z_t = [x_{t-N+1},\ldots,x_{t}],
\]
then compute the matrix $D_t$ and $G_t$ following \cref{def:matrices_2}, see \cref{alg:forward_estimate} for the detailed implementation.



This method present several advantages: it ensure good theoretical performance, especially since $\kappa=1$ (see \cref{thm:forward_estimate_properties}), at the cost of only one extra gradient evaluation.

\begin{theorem}\label{thm:forward_estimate_properties}
    The \textit{``orthogonal forward estimate only''} update described in \cref{alg:forward_estimate} satisfies \cref{assump:bounded_conditionning,assump:projector_grad} with $\kappa = 1$.
\end{theorem}


\subsubsection{"Random Orthogonal Directions" update rule}

The "Random Orthogonal Direction" update consists in creating a batch of $N$ random orthogonal direction at each iteration, such that
\[
    \mathbb{E}[D_tD_t^T] = \frac{N}{d}I.
\]
For instance, $D_t$ could be the $Q$ matrix of a \texttt{qr} decomposition of a random $N\times d$ matrix (complexity: $O(N^2 d)$), or even simpler, be an aggregation of random canonical vectors (see e.g. \cite{hanzely2020stochastic}).

Afterward, it remains to update the matrices $Y_t,\, Z_t, G_t$ as follow,
\[
    Z_t = [x_t,\ldots, x_t], \quad Y_t = Z_t + hD_t, \quad G_t = \cref{def:matrices_2}.
\]
See \cref{alg:ortho_random} for the detailed implementation. The major advantage of this approach is that $\kappa = 1$ and $\delta = \sqrt{N}\cdot h$. However, $N$ additional gradient computations are required to create the matrix $G_t$.


\subsubsection{Other Matrix Updates: Pruning or Orthogonalization} 


It is possible to create other kind of matrix updates, for instance, the \textit{Iterates only} (stores only the last forward estimate and previous iterates) or \textit{Greedy} (stores all previous forward estimates \textit{and} iterates) strategies, detailed below:
\begin{align}
    Y_{t} &= [x_{t+\frac{1}{2}}, x_t, x_{t-1},\ldots, x_{t-N+2}], \quad  Z_{t} = [x_t, x_{t-1},\ldots, x_{t-N+1}] \tag{Iterates only}\\
    Y_{t} &= [x_{t+\frac{1}{2}}, x_{t},x_{t-\frac{1}{2}},\ldots, x_{t-\frac{N+2}{2}}],\quad Z_{t} = [x_{t},x_{t-\frac{1}{2}},\ldots, x_{t-\frac{N+1}{2}}] \tag{Greedy}
\end{align}
However, it is impossible to ensure that the directions in $D_t$ will be orthogonal, hence $\kappa$ in \cref{assump:bounded_conditionning} might be huge. Nevertheless, it is possible to bound the condition number by pruning or via an orthogonalization procedure.


\paragraph{Pruning.} It suffices to check the condition number of $D_t$, then prune the columns of $Y_t,\, Z_t,\, D_t,\,\text{and } G_t$ until $\kappa$ is sufficiently small, for instance, until $\kappa\leq 10^3$. Note that, by the nature of those matrices, their condition number grows quickly \cite{tyrtyshnikov1994bad,scieur2016regularized}, hence the number of resulting column might be small.

\paragraph{Orthogonalization} From the matrices $Y_t,\, Z_t$, the matrix $D_t$ is computed as $D_t = \texttt{qr}(Z_t-Y_t)$. Then, the rest of the procedure follows the same steps as the "Random Orthogonal Directions" rule.

The pruning strategy is cheaper than the orthogonalization, at the cost of losing control on how large the history is. The  orthogonalization technique present the same advantages as the "Random Orthogonal Directions" rule, but the directions taken might me more relevant than random ones.






==> update_matrix.tex <==

\section{Some update strategies for matrices \texorpdfstring{$Y,\,Z,\,D,\,G$}{Y, Z, D, G}} 

The framework presented in this paper is characterized by its generality, requiring only minimal assumptions on the matrix $D$ and vector $\varepsilon$. This section explores different strategies for updating the matrices from \cref{def:matrices}, which can be classified into two categories: \textit{online} and \textit{batch techniques}.

\textbf{Recommended method.} Among all the methods presented in this section, the most promising technique seems to be the \textit{Orthogonal Forward Estimates Only}, as it ensures that the condition number $\kappa_D = 1$ and the norm of the error vector $\|\varepsilon\|$ is small.


\subsection{Online Techniques}

The online technique updates the matrix $D$ while \cref{alg:type1_iterative,alg:accelerated_algo_sketch} are running. To achieve \cref{assump:projector_grad}, the method employs either a steepest or orthogonal forward estimate, defined as
\[
x_{t+\frac{1}{2}} = x_t - h \nabla f(x_t) \quad \textit{(steepest)} \quad \text{or} \quad x_{t+\frac{1}{2}} = x_t - h(I-P_{t-1})\frac{\nabla f(x_t)}{\|\nabla f(x_t)\|} \quad \textit{(orthogonal)}.
\]
Then, it include $x_{t+\frac{1}{2}}-x_t$ in the matrix $D_t$. The projector $P_{t-1}$ is defined in \cref{def:p_projector}, and parameter $h$ can be a fixed small value (e.g., $h = 10^{-9}$). This section investigates three different strategies for storing past information: \textit{Iterates only}, \textit{Forward Estimates Only}, and \textit{Greedy}, listed below.
\begin{align}
    Y_{t} &= [x_{t+\frac{1}{2}}, x_t, x_{t-1},\ldots, x_{t-N+2}], \quad  Z_{t} = [x_t, x_{t-1},\ldots, x_{t-N+1}] \tag{Iterates only}\\
    Y_{t} &= [x_{t+\frac{1}{2}}, x_{t-\frac{1}{2}},\ldots, , x_{t-N+\frac{3}{2}}],  \quad Z_{t} = [x_t, x_{t-1}, \ldots, x_{t-N+1}] \tag{Forward Estimates Only}\\
    Y_{t} &= [x_{t+\frac{1}{2}}, x_{t},x_{t-\frac{1}{2}},\ldots, x_{t-\frac{N+2}{2}}],\quad Z_{t} = [x_{t},x_{t-\frac{1}{2}},\ldots, x_{t-\frac{N+1}{2}}] \tag{Greedy}
\end{align}


\textbf{Iterates only:} In the case of quasi-Newton updates and Nonlinear/Anderson acceleration, the iterates are constructed using the equation $x_{t+1}-x_t\in \nabla f(x_t)+ \textbf{span}\{x_{t-i+1}-x_{t-i}\}_{i=1\ldots N}$. The update draws inspiration from this observation. However, it does not provide control over the condition number of $D_t$ or the norm $\|\varepsilon\|$. To address this, one can either accept a potentially high condition number or remove the oldest points in $D$ and $G$ until the condition number is bounded (e.g., $\kappa = 10^9$).

\textbf{Forward Estimates Only:} This method provides more control over the iterates added to $Y$ and $Z$. When using the \textit{orthogonal} technique to compute $x_{i+\frac{1}{2}}$ reduces the constants in \cref{thm:rate_nonconvex,thm:rate_starconvex,thm:rate_acc_sketch}: the condition number of $D$ is equal to 1 as $D^TD = h^2I$, and the norm of $\varepsilon$ is small ($\|\varepsilon\| \leq O(h)$).

\textbf{Greedy:} The greedy approach involves storing both the iterates and the forward approximations. It shares the same drawback as the \textit{Iterates only} strategy but retains at least the most recent information about the Hessian-vector product approximation, thereby reducing the $\|z_i-x_{i}\|$ term in $\varepsilon$ \eqref{eq:error_vector}.


\subsection{Batch Techniques}

Instead of making individual updates, an alternative approach is to compute them collectively, centered on $x_t$. This technique generates a matrix $D_t$ consisting of $N$ orthogonal directions $d_1, \cdots, d_N$ of norm $h$.  The corresponding $Y_t, Z_t, G_t$ matrices are then defined as follows:
\[
    Y_t = [x_t+d_1,\ldots, x_t+d_n], \quad Z_t = [x_t,\ldots,x_t], \quad G_t = [\ldots, \nabla f(x_t+d_i)-\nabla f(x_t),\ldots].
\]
This section explores two batch techniques that generate orthogonal directions: \textit{Orthogonalization} and \textit{Random Subspace}. Both lead to $\delta = 3h$ and $\kappa = 1$ in \cref{assump:bounded_epsilon,assump:bounded_conditionning}. However, they require $N$ additional gradient computations at each iteration (instead of one for the online techniques). For clarity, in the experiments, only the Greedy version is considered.

\paragraph{Orthogonalization:} This technique involves using any online technique discussed in the previous section and storing the directions in a matrix $\tilde D_t$. Then, it constructs the matrices $D_t$ by performing an orthogonalization procedure on $\tilde D_t$, such as the QR algorithm. This approach provides Hessian estimates in relevant directions, which can be more beneficial than random ones.

\paragraph{Random Subspace:} Inspired by \citep{hanzely2020stochastic}, this technique randomly generates $D_t$ at each iteration by either taking $D_t$ to be $N$ random (rescaled) canonical vectors or by using the $Q$ matrix from the QR decomposition of a random $N\times D$ matrix. This ensures that $D_t$ satisfies \cref{assump:random_projector}. For clarity, in the experiments, only the QR version is considered.



